Written Justifications are Key to Aggregate Crowdsourced Forecasts

This paper demonstrates that aggregating crowdsourced forecasts benefits from modeling the written justifications provided by forecasters. Our experiments show that the majority and weighted vote baselines are competitive, and that the written justifications are beneficial to call a question throughout its life except in the last quarter. We also conduct an error analysis shedding light into the characteristics that make a justification unreliable.

==> figures/nn.tex <==
\vspace{2.5in}

==> tables/extraresults.tex <==
\newcommand{\sintra}{$^{\dagger}$}
\newcommand{\sinter}{$^{\ddagger}$}
%\setlength{\tabcolsep}{.08in}
\begin{tabular}{l @{\hspace{.5in}} r@{}l @{\hspace{.5in}} c@{}l c@{}l c@{}l c@{}l}
\toprule
& \multicolumn{9}{c}{question difficulty (according to best baseline)} \\ \cmidrule{2-10}
& All && Q1 && Q2 && Q3 && Q4 \\ \midrule


Using daily forecasts only \\
~~~~~~Baselines \\
~~~~~~~~~~~~Majority vote (predictions)
&71.89& & 95.52 && 86.62 && 73.14 && 32.73 \\
~~~~~~~~~~~~Weighted vote (predictions)
&73.79&  & 97.61 && 89.02 && 75.09 && 33.89 \\

~~~~~~Neural network with components \ldots \\
~~~~~~~~~~~~predictions
&77.96&\sintra& 92.96 &\sintra&  78.16 &\sintra& 70.58 &\sintra& 69.77&\sintra \\
~~~~~~~~~~~~predictions + question
&77.61&\sintra& 97.44 &\sinter&  83.2 &\sintra\sinter& 76.49 &\sinter& 53.34&\sintra\sinter \\
~~~~~~~~~~~~predictions + justifications
&80.23&\sintra\sinter& 96.45 &\sintra\sinter&  86.74 &\sintra\sinter& 77.71 &\sintra\sinter& 60.04&\sintra\sinter \\
~~~~~~~~~~~~predictions + question + justifications
&79.96&\sintra\sinter& 96.51 &\sintra\sinter& 86.50 &\sintra\sinter& 78.92 &\sintra\sinter& 58.00&\sintra\sinter \\ \midrule

Using active forecasts \\
~~~~~~Baselines \\
~~~~~~~~~~~~Majority vote (predictions)
&77.27&  & 98.75 && 99.35 && 86.35 && 26.91 \\
~~~~~~~~~~~~Weighted vote (predictions)
&77.97&  & 99.40 && 99.55 && 86.01 && 29.30 \\

~~~~~~Neural network with components \ldots \\
~~~~~~~~~~~~predictions
&78.81&  & 89.53 &\sintra&  85.09 &\sintra& 74.55 &\sintra& 68.24&\sintra \\
~~~~~~~~~~~~predictions + question
&79.35&\sintra  & 94.58 &\sintra\sinter&  88.01 &\sintra\sinter& 78.04 &\sintra\sinter& 58.73&\sintra\sinter \\
~~~~~~~~~~~~predictions + justifications
&80.84&\sintra\sinter  & 95.71 &\sintra\sinter& 93.18 &\sintra\sinter& 79.99 &\sintra\sinter&  57.05&\sintra\sinter \\
~~~~~~~~~~~~predictions + question + justifications
&81.27&\sintra\sinter  & 94.17 &\sintra\sinter& 90.11 &\sintra\sinter& 78.67 &\sintra\sinter& 64.41&\sintra\sinter \\

\bottomrule

\end{tabular}

